Autoregressive Dynamics Models for Offline Policy Evaluation and Optimization

Standard dynamics models for continuous control make use of feedforward computation to predict the conditional distribution of next state and reward given current state and action using a multivariate Gaussian with a diagonal covariance structure. This modeling choice assumes that different dimensions of the next state and reward are conditionally independent given the current state and action and may be driven by the fact that fully observable physics-based simulation environments entail deterministic transition dynamics. In this paper, we challenge this conditional independence assumption and propose a family of expressive autoregressive dynamics models that generate different dimensions of the next state and reward sequentially conditioned on previous dimensions. We demonstrate that autoregressive dynamics models indeed outperform standard feedforward models in log-likelihood on heldout transitions. Furthermore, we compare different model-based and model-free off-policy evaluation (OPE) methods on RL Unplugged, a suite of offline MuJoCo datasets, and find that autoregressive dynamics models consistently outperform all baselines, achieving a new state-of-the-art. Finally, we show that autoregressive dynamics models are useful for offline policy optimization by serving as a way to enrich the replay buffer through data augmentation and improving performance using model-based planning.

==> tables/absolute_error_table.tex <==
\begin{table} \begin{center}
\small
 \begin{tabular}{@{\hspace{.2cm}}l@{\hspace{.1cm}}l@{\hspace{.3cm}}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.2cm}}}
 \toprule
& &\multirow{2}{*}{}  & \multicolumn{2}{c}{Cartpole} & \multicolumn{2}{c}{Cheetah} & \multicolumn{2}{c}{Finger} & \multicolumn{2}{c}{Fish} & \multicolumn{2}{c}{Humanoid}\\
& &  & \multicolumn{2}{c}{swingup} & \multicolumn{2}{c}{run} & \multicolumn{2}{c}{turn hard} & \multicolumn{2}{c}{swim} & \multicolumn{2}{c}{run}\\
\midrule
\multirow{8}{*}{\rotatebox{90}{{\bf Absolute Error} btw.}} & \multirow{8}{*}{\rotatebox{90}{OPE and ground truth}} & Variational power method &$\color{dgray} 37.53$ & $\color{dgray} {\scriptstyle \, \pm 3.50}$ & $\color{dgray} 61.89$ & $\color{dgray} {\scriptstyle \, \pm 4.25}$ & $\color{dgray} 46.22$ & $\color{dgray} {\scriptstyle \, \pm 3.93}$ & $\color{dgray} 31.27$ & $\color{dgray} {\scriptstyle \, \pm 0.99}$ & $\color{dgray} 35.29$ & $\color{dgray} {\scriptstyle \, \pm 3.03}$\\
& & Importance Sampling &$\color{dgray} 68.75$ & $\color{dgray} {\scriptstyle \, \pm 2.39}$ & $\color{dgray} 44.29$ & $\color{dgray} {\scriptstyle \, \pm 1.91}$ & $\color{dgray} 90.10$ & $\color{dgray} {\scriptstyle \, \pm 4.68}$ & $\color{dgray} 34.82$ & $\color{dgray} {\scriptstyle \, \pm 1.93}$ & $\color{dgray} 27.89$ & $\color{dgray} {\scriptstyle \, \pm 1.98}$\\
& & Best DICE &$\color{dgray} 22.73$ & $\color{dgray} {\scriptstyle \, \pm 1.65}$ & $\color{dgray} 23.35$ & $\color{dgray} {\scriptstyle \, \pm 1.32}$ & $\color{dgray} 33.52$ & $\color{dgray} {\scriptstyle \, \pm 3.48}$ & $\color{dgray} 59.48$ & $\color{dgray} {\scriptstyle \, \pm 2.47}$ & $\color{dgray} 31.42$ & $\color{dgray} {\scriptstyle \, \pm 2.04}$\\
& & Feedforward Model &$\bf 6.80$ & $\bf {\scriptstyle \, \pm 0.85}$ & $\color{dgray} 13.64$ & $\color{dgray} {\scriptstyle \, \pm 0.59}$ & $\color{dgray} 35.99$ & $\color{dgray} {\scriptstyle \, \pm 3.00}$ & $\bf 4.75$ & $\bf {\scriptstyle \, \pm 0.23}$ & $\color{dgray} 30.12$ & $\color{dgray} {\scriptstyle \, \pm 2.40}$\\
& & FQE (L2) &$\color{dgray} 19.02$ & $\color{dgray} {\scriptstyle \, \pm 1.34}$ & $\color{dgray} 48.26$ & $\color{dgray} {\scriptstyle \, \pm 1.78}$ & $\color{dgray} 27.91$ & $\color{dgray} {\scriptstyle \, \pm 1.18}$ & $\color{dgray} 19.82$ & $\color{dgray} {\scriptstyle \, \pm 1.57}$ & $\color{dgray} 56.28$ & $\color{dgray} {\scriptstyle \, \pm 3.52}$\\
& & Doubly Robust (IS, FQE) &$\color{dgray} 24.38$ & $\color{dgray} {\scriptstyle \, \pm 2.51}$ & $\color{dgray} 40.27$ & $\color{dgray} {\scriptstyle \, \pm 2.05}$ & $\color{dgray} 25.26$ & $\color{dgray} {\scriptstyle \, \pm 2.48}$ & $\color{dgray} 20.28$ & $\color{dgray} {\scriptstyle \, \pm 1.90}$ & $\color{dgray} 53.64$ & $\color{dgray} {\scriptstyle \, \pm 3.68}$\\
& & FQE (distributional) &$\color{dgray} 12.63$ & $\color{dgray} {\scriptstyle \, \pm 1.21}$ & $\color{dgray} 36.50$ & $\color{dgray} {\scriptstyle \, \pm 1.62}$ & $\bf 10.23$ & $\bf {\scriptstyle \, \pm 0.93}$ & $\color{dgray} 7.76$ & $\color{dgray} {\scriptstyle \, \pm 0.95}$ & $\color{dgray} 32.36$ & $\color{dgray} {\scriptstyle \, \pm 2.27}$\\
& & Autoregressive Model &$\bf 5.32$ & $\bf {\scriptstyle \, \pm 0.54}$ & $\bf 4.64$ & $\bf {\scriptstyle \, \pm 0.46}$ & $\color{dgray} 22.93$ & $\color{dgray} {\scriptstyle \, \pm 1.72}$ & $\bf 4.31$ & $\bf {\scriptstyle \, \pm 0.22}$ & $\bf 20.95$ & $\bf {\scriptstyle \, \pm 1.61}$\\
\midrule
\midrule
& & \multirow{2}{*}{}  & \multicolumn{2}{c}{Walker} & \multicolumn{2}{c}{Walker} & \multicolumn{2}{c}{Manipulator} & \multicolumn{2}{c}{Manipulator} & \multicolumn{2}{c}{\multirow{2}{*}{Median $\downarrow$}}\\
& &  & \multicolumn{2}{c}{stand} & \multicolumn{2}{c}{walk} & \multicolumn{2}{c}{insert ball} & \multicolumn{2}{c}{insert peg}\\
\midrule
\multirow{8}{*}{\rotatebox{90}{{\bf Absolute Error} btw.}} & \multirow{8}{*}{\rotatebox{90}{OPE and ground truth}} & Variational power method &$\color{dgray} 96.76$ & $\color{dgray} {\scriptstyle \, \pm 3.59}$ & $\color{dgray} 87.24$ & $\color{dgray} {\scriptstyle \, \pm 4.25}$ & $\color{dgray} 79.25$ & $\color{dgray} {\scriptstyle \, \pm 6.19}$ & $\color{dgray} 21.95$ & $\color{dgray} {\scriptstyle \, \pm 1.17}$ & \multicolumn{2}{c}{$46.22$}\\
& & Importance Sampling &$\color{dgray} 66.50$ & $\color{dgray} {\scriptstyle \, \pm 1.90}$ & $\color{dgray} 67.24$ & $\color{dgray} {\scriptstyle \, \pm 2.70}$ & $\color{dgray} 29.93$ & $\color{dgray} {\scriptstyle \, \pm 1.10}$ & $\color{dgray} 12.78$ & $\color{dgray} {\scriptstyle \, \pm 0.66}$ & \multicolumn{2}{c}{$44.29$}\\
& & Best DICE &$\color{dgray} 27.58$ & $\color{dgray} {\scriptstyle \, \pm 3.01}$ & $\color{dgray} 47.28$ & $\color{dgray} {\scriptstyle \, \pm 3.13}$ & $\color{dgray} 103.45$ & $\color{dgray} {\scriptstyle \, \pm 5.21}$ & $\color{dgray} 22.75$ & $\color{dgray} {\scriptstyle \, \pm 3.00}$ & \multicolumn{2}{c}{$31.42$}\\
& & Feedforward Model &$\color{dgray} 23.34$ & $\color{dgray} {\scriptstyle \, \pm 2.41}$ & $\color{dgray} 52.23$ & $\color{dgray} {\scriptstyle \, \pm 2.34}$ & $\color{dgray} 34.30$ & $\color{dgray} {\scriptstyle \, \pm 2.55}$ & $\color{dgray} 121.12$ & $\color{dgray} {\scriptstyle \, \pm 1.58}$ & \multicolumn{2}{c}{$30.12$}\\
& & FQE (L2) &$\bf 6.51$ & $\bf {\scriptstyle \, \pm 0.71}$ & $\color{dgray} 18.34$ & $\color{dgray} {\scriptstyle \, \pm 0.95}$ & $\color{dgray} 36.32$ & $\color{dgray} {\scriptstyle \, \pm 1.07}$ & $\color{dgray} 31.12$ & $\color{dgray} {\scriptstyle \, \pm 2.37}$ & \multicolumn{2}{c}{$27.91$}\\
& & Doubly Robust (IS, FQE) &$\color{dgray} 26.82$ & $\color{dgray} {\scriptstyle \, \pm 2.66}$ & $\color{dgray} 24.63$ & $\color{dgray} {\scriptstyle \, \pm 1.69}$ & $\color{dgray} 13.33$ & $\color{dgray} {\scriptstyle \, \pm 1.16}$ & $\color{dgray} 22.28$ & $\color{dgray} {\scriptstyle \, \pm 2.34}$ & \multicolumn{2}{c}{$24.63$}\\
& & FQE (distributional) &$\color{dgray} 21.49$ & $\color{dgray} {\scriptstyle \, \pm 1.41}$ & $\color{dgray} 27.57$ & $\color{dgray} {\scriptstyle \, \pm 1.54}$ & $\bf 9.75$ & $\bf {\scriptstyle \, \pm 1.10}$ & $\color{dgray} 12.66$ & $\color{dgray} {\scriptstyle \, \pm 1.39}$ & \multicolumn{2}{c}{$12.66$}\\
& & Autoregressive Model &$\color{dgray} 19.12$ & $\color{dgray} {\scriptstyle \, \pm 1.23}$ & $\bf 5.14$ & $\bf {\scriptstyle \, \pm 0.49}$ & $\color{dgray} 17.13$ & $\color{dgray} {\scriptstyle \, \pm 1.34}$ & $\bf 9.71$ & $\bf {\scriptstyle \, \pm 0.70}$ & \multicolumn{2}{c}{$9.71$}\\
 \bottomrule
 \end{tabular}
\caption{\label{tab:abs-error} \small Average absolute error between OPE metrics and ground truth values at a discount factor of 0.995.
In each column, absolute error values that are not significantly different from the best ($p > 0.05$) are bold faced. Methods are ordered by median.}
\end{center}  \end{table}

==> tables/rank_correlation_table.tex <==
\begin{table} \begin{center}
\small
 \begin{tabular}{@{\hspace{.2cm}}l@{\hspace{.1cm}}l@{\hspace{.3cm}}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.2cm}}}
 \toprule
& &\multirow{2}{*}{}  & \multicolumn{2}{c}{Cartpole} & \multicolumn{2}{c}{Cheetah} & \multicolumn{2}{c}{Finger} & \multicolumn{2}{c}{Fish} & \multicolumn{2}{c}{Humanoid}\\
& &  & \multicolumn{2}{c}{swingup} & \multicolumn{2}{c}{run} & \multicolumn{2}{c}{turn hard} & \multicolumn{2}{c}{swim} & \multicolumn{2}{c}{run}\\
\midrule
\multirow{8}{*}{\rotatebox{90}{ Rank Correlation btw.}} & \multirow{8}{*}{\rotatebox{90}{OPE and ground truth}} & Importance Sampling &$\color{dgray} -0.23$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\color{dgray} -0.01$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$ & $\color{dgray} -0.45$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$ & $\color{dgray} -0.17$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\bf 0.91$ & $\bf {\scriptstyle \, \pm 0.02}$\\
& & Best DICE &$\color{dgray} -0.16$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\color{dgray} 0.07$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\color{dgray} -0.22$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\color{dgray} 0.44$ & $\color{dgray} {\scriptstyle \, \pm 0.09}$ & $\color{dgray} -0.10$ & $\color{dgray} {\scriptstyle \, \pm 0.10}$\\
& & Variational power method &$\color{dgray} 0.01$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\color{dgray} 0.01$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$ & $\color{dgray} -0.25$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\color{dgray} 0.56$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$ & $\color{dgray} 0.36$ & $\color{dgray} {\scriptstyle \, \pm 0.09}$\\
& & Doubly Robust (IS, FQE) &$\color{dgray} 0.55$ & $\color{dgray} {\scriptstyle \, \pm 0.09}$ & $\color{dgray} 0.56$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$ & $\color{dgray} 0.67$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\color{dgray} 0.11$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$ & $\color{dgray} -0.03$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$\\
& & Feedforward Model &$\color{dgray} 0.83$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\bf 0.64$ & $\bf {\scriptstyle \, \pm 0.08}$ & $\color{dgray} 0.08$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\bf 0.95$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\color{dgray} 0.35$ & $\color{dgray} {\scriptstyle \, \pm 0.10}$\\
& & FQE (distributional) &$\color{dgray} 0.69$ & $\color{dgray} {\scriptstyle \, \pm 0.07}$ & $\bf 0.67$ & $\bf {\scriptstyle \, \pm 0.06}$ & $\bf 0.94$ & $\bf {\scriptstyle \, \pm 0.01}$ & $\color{dgray} 0.59$ & $\color{dgray} {\scriptstyle \, \pm 0.10}$ & $\color{dgray} 0.74$ & $\color{dgray} {\scriptstyle \, \pm 0.06}$\\
& & FQE (L2) &$\color{dgray} 0.70$ & $\color{dgray} {\scriptstyle \, \pm 0.07}$ & $\color{dgray} 0.56$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$ & $\color{dgray} 0.83$ & $\color{dgray} {\scriptstyle \, \pm 0.04}$ & $\color{dgray} 0.10$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$ & $\color{dgray} -0.02$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$\\
& & Autoregressive Model &$\bf 0.91$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\bf 0.74$ & $\bf {\scriptstyle \, \pm 0.07}$ & $\color{dgray} 0.57$ & $\color{dgray} {\scriptstyle \, \pm 0.09}$ & $\bf 0.96$ & $\bf {\scriptstyle \, \pm 0.01}$ & $\bf 0.90$ & $\bf {\scriptstyle \, \pm 0.02}$\\
\midrule
\midrule
& & \multirow{2}{*}{}  & \multicolumn{2}{c}{Walker} & \multicolumn{2}{c}{Walker} & \multicolumn{2}{c}{Manipulator} & \multicolumn{2}{c}{Manipulator} & \multicolumn{2}{c}{\multirow{2}{*}{Median $\uparrow$}}\\
& &  & \multicolumn{2}{c}{stand} & \multicolumn{2}{c}{walk} & \multicolumn{2}{c}{insert ball} & \multicolumn{2}{c}{insert peg}\\
\midrule
\multirow{8}{*}{\rotatebox{90}{ Rank Correlation btw.}} & \multirow{8}{*}{\rotatebox{90}{OPE and ground truth}} & Importance Sampling &$\color{dgray} 0.59$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$ & $\color{dgray} 0.38$ & $\color{dgray} {\scriptstyle \, \pm 0.10}$ & $\color{dgray} -0.72$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\color{dgray} -0.25$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$ & \multicolumn{2}{c}{$-0.17$}\\
& & Best DICE &$\color{dgray} -0.11$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$ & $\color{dgray} -0.58$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$ & $\color{dgray} 0.19$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\color{dgray} -0.35$ & $\color{dgray} {\scriptstyle \, \pm 0.10}$ & \multicolumn{2}{c}{$-0.11$}\\
& & Variational power method &$\color{dgray} -0.35$ & $\color{dgray} {\scriptstyle \, \pm 0.10}$ & $\color{dgray} -0.10$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\bf 0.61$ & $\bf {\scriptstyle \, \pm 0.08}$ & $\bf 0.41$ & $\bf {\scriptstyle \, \pm 0.09}$ & \multicolumn{2}{c}{$0.01$}\\
& & Doubly Robust (IS, FQE) &$\color{dgray} 0.88$ & $\color{dgray} {\scriptstyle \, \pm 0.03}$ & $\color{dgray} 0.85$ & $\color{dgray} {\scriptstyle \, \pm 0.04}$ & $\color{dgray} 0.42$ & $\color{dgray} {\scriptstyle \, \pm 0.10}$ & $\color{dgray} -0.47$ & $\color{dgray} {\scriptstyle \, \pm 0.09}$ & \multicolumn{2}{c}{$0.55$}\\
& & Feedforward Model &$\color{dgray} 0.82$ & $\color{dgray} {\scriptstyle \, \pm 0.04}$ & $\color{dgray} 0.80$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\color{dgray} 0.06$ & $\color{dgray} {\scriptstyle \, \pm 0.10}$ & $\color{dgray} -0.56$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$ & \multicolumn{2}{c}{$0.64$}\\
& & FQE (distributional) &$\color{dgray} 0.87$ & $\color{dgray} {\scriptstyle \, \pm 0.02}$ & $\color{dgray} 0.89$ & $\color{dgray} {\scriptstyle \, \pm 0.03}$ & $\bf 0.63$ & $\bf {\scriptstyle \, \pm 0.08}$ & $\color{dgray} -0.23$ & $\color{dgray} {\scriptstyle \, \pm 0.10}$ & \multicolumn{2}{c}{$0.69$}\\
& & FQE (L2) &$\bf 0.96$ & $\bf {\scriptstyle \, \pm 0.01}$ & $\color{dgray} 0.94$ & $\color{dgray} {\scriptstyle \, \pm 0.02}$ & $\bf 0.70$ & $\bf {\scriptstyle \, \pm 0.07}$ & $\color{dgray} -0.48$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$ & \multicolumn{2}{c}{$0.70$}\\
& & Autoregressive Model &$\bf 0.96$ & $\bf {\scriptstyle \, \pm 0.01}$ & $\bf 0.98$ & $\bf {\scriptstyle \, \pm 0.00}$ & $\color{dgray} -0.33$ & $\color{dgray} {\scriptstyle \, \pm 0.09}$ & $\bf 0.47$ & $\bf {\scriptstyle \, \pm 0.09}$ & \multicolumn{2}{c}{$0.90$}\\
 \bottomrule
 \end{tabular}
\caption{\label{tab:rank} \small Spearman's rank correlation ($\rho$) coefficient (bootstrap mean $\pm$ standard deviation)
between different OPE metrics and ground truth values at a discount factor of $0.995$.
In each column, rank correlation coefficients that are not significantly different from the best ($p >0.05$) are bold faced.
Methods are ordered by median. Also see \tabref{tab:regret5} and \tabref{tab:abs-error} for Normalized Regret@5 and Average Absolute Error results.}
\end{center}  \end{table}

==> tables/regret_table.tex <==
\begin{table} \begin{center}
\small
 \begin{tabular}{@{\hspace{.2cm}}l@{\hspace{.1cm}}l@{\hspace{.3cm}}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.3cm}}r@{}l@{\hspace{.2cm}}}
 \toprule
& &\multirow{2}{*}{}  & \multicolumn{2}{c}{Cartpole} & \multicolumn{2}{c}{Cheetah} & \multicolumn{2}{c}{Finger} & \multicolumn{2}{c}{Fish} & \multicolumn{2}{c}{Humanoid}\\
& &  & \multicolumn{2}{c}{swingup} & \multicolumn{2}{c}{run} & \multicolumn{2}{c}{turn hard} & \multicolumn{2}{c}{swim} & \multicolumn{2}{c}{run}\\
\midrule
\multirow{8}{*}{\rotatebox{90}{{\bf Regret@5} for}} & \multirow{8}{*}{\rotatebox{90}{OPE \vs{} ground truth}} & Importance Sampling &$\color{dgray} 0.73$ & $\color{dgray} {\scriptstyle \, \pm 0.16}$ & $\color{dgray} 0.40$ & $\color{dgray} {\scriptstyle \, \pm 0.21}$ & $\color{dgray} 0.64$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\color{dgray} 0.12$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\bf 0.31$ & $\bf {\scriptstyle \, \pm 0.09}$\\
& & Best DICE &$\color{dgray} 0.68$ & $\color{dgray} {\scriptstyle \, \pm 0.41}$ & $\color{dgray} 0.27$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\color{dgray} 0.44$ & $\color{dgray} {\scriptstyle \, \pm 0.04}$ & $\bf 0.35$ & $\bf {\scriptstyle \, \pm 0.24}$ & $\color{dgray} 0.84$ & $\color{dgray} {\scriptstyle \, \pm 0.22}$\\
& & Variational power method &$\color{dgray} 0.50$ & $\color{dgray} {\scriptstyle \, \pm 0.13}$ & $\color{dgray} 0.37$ & $\color{dgray} {\scriptstyle \, \pm 0.04}$ & $\color{dgray} 0.45$ & $\color{dgray} {\scriptstyle \, \pm 0.13}$ & $\bf 0.02$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\color{dgray} 0.56$ & $\color{dgray} {\scriptstyle \, \pm 0.08}$\\
& & Doubly Robust (IS, FQE) &$\color{dgray} 0.28$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\bf 0.09$ & $\bf {\scriptstyle \, \pm 0.05}$ & $\color{dgray} 0.56$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$ & $\color{dgray} 0.61$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$ & $\color{dgray} 0.99$ & $\color{dgray} {\scriptstyle \, \pm 0.00}$\\
& & FQE (L2) &$\color{dgray} 0.06$ & $\color{dgray} {\scriptstyle \, \pm 0.04}$ & $\color{dgray} 0.17$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\bf 0.30$ & $\bf {\scriptstyle \, \pm 0.11}$ & $\color{dgray} 0.50$ & $\color{dgray} {\scriptstyle \, \pm 0.03}$ & $\color{dgray} 0.99$ & $\color{dgray} {\scriptstyle \, \pm 0.00}$\\
& & Feedforward Model &$\bf 0.02$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\color{dgray} 0.24$ & $\color{dgray} {\scriptstyle \, \pm 0.12}$ & $\color{dgray} 0.43$ & $\color{dgray} {\scriptstyle \, \pm 0.04}$ & $\bf 0.00$ & $\bf {\scriptstyle \, \pm 0.00}$ & $\color{dgray} 0.44$ & $\color{dgray} {\scriptstyle \, \pm 0.02}$\\
& & FQE (distributional) &$\bf 0.03$ & $\bf {\scriptstyle \, \pm 0.09}$ & $\bf 0.11$ & $\bf {\scriptstyle \, \pm 0.09}$ & $\bf 0.10$ & $\bf {\scriptstyle \, \pm 0.12}$ & $\color{dgray} 0.49$ & $\color{dgray} {\scriptstyle \, \pm 0.06}$ & $\bf 0.24$ & $\bf {\scriptstyle \, \pm 0.15}$\\
& & Autoregressive Model &$\bf 0.00$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\bf 0.01$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\color{dgray} 0.63$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\bf 0.03$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\bf 0.32$ & $\bf {\scriptstyle \, \pm 0.06}$\\
\midrule
\midrule
& & \multirow{2}{*}{}  & \multicolumn{2}{c}{Walker} & \multicolumn{2}{c}{Walker} & \multicolumn{2}{c}{Manipulator} & \multicolumn{2}{c}{Manipulator} & \multicolumn{2}{c}{\multirow{2}{*}{Median $\downarrow$}}\\
& &  & \multicolumn{2}{c}{stand} & \multicolumn{2}{c}{walk} & \multicolumn{2}{c}{insert ball} & \multicolumn{2}{c}{insert peg}\\
\midrule
\multirow{8}{*}{\rotatebox{90}{{\bf Regret@5} for}} & \multirow{8}{*}{\rotatebox{90}{OPE \vs{} ground truth}} & Importance Sampling &$\color{dgray} 0.54$ & $\color{dgray} {\scriptstyle \, \pm 0.11}$ & $\color{dgray} 0.54$ & $\color{dgray} {\scriptstyle \, \pm 0.23}$ & $\color{dgray} 0.83$ & $\color{dgray} {\scriptstyle \, \pm 0.05}$ & $\bf 0.22$ & $\bf {\scriptstyle \, \pm 0.03}$ & \multicolumn{2}{c}{$0.54$}\\
& & Best DICE &$\color{dgray} 0.24$ & $\color{dgray} {\scriptstyle \, \pm 0.07}$ & $\color{dgray} 0.55$ & $\color{dgray} {\scriptstyle \, \pm 0.06}$ & $\bf 0.44$ & $\bf {\scriptstyle \, \pm 0.07}$ & $\color{dgray} 0.75$ & $\color{dgray} {\scriptstyle \, \pm 0.04}$ & \multicolumn{2}{c}{$0.44$}\\
& & Variational power method &$\color{dgray} 0.41$ & $\color{dgray} {\scriptstyle \, \pm 0.02}$ & $\color{dgray} 0.39$ & $\color{dgray} {\scriptstyle \, \pm 0.02}$ & $\bf 0.52$ & $\bf {\scriptstyle \, \pm 0.20}$ & $\color{dgray} 0.32$ & $\color{dgray} {\scriptstyle \, \pm 0.02}$ & \multicolumn{2}{c}{$0.41$}\\
& & Doubly Robust (IS, FQE) &$\bf 0.02$ & $\bf {\scriptstyle \, \pm 0.01}$ & $\bf 0.05$ & $\bf {\scriptstyle \, \pm 0.07}$ & $\bf 0.30$ & $\bf {\scriptstyle \, \pm 0.10}$ & $\color{dgray} 0.73$ & $\color{dgray} {\scriptstyle \, \pm 0.01}$ & \multicolumn{2}{c}{$0.30$}\\
& & FQE (L2) &$\bf 0.04$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\bf 0.00$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\bf 0.37$ & $\bf {\scriptstyle \, \pm 0.07}$ & $\color{dgray} 0.74$ & $\color{dgray} {\scriptstyle \, \pm 0.01}$ & \multicolumn{2}{c}{$0.30$}\\
& & Feedforward Model &$\bf 0.18$ & $\bf {\scriptstyle \, \pm 0.10}$ & $\bf 0.03$ & $\bf {\scriptstyle \, \pm 0.05}$ & $\color{dgray} 0.83$ & $\color{dgray} {\scriptstyle \, \pm 0.06}$ & $\color{dgray} 0.74$ & $\color{dgray} {\scriptstyle \, \pm 0.01}$ & \multicolumn{2}{c}{$0.24$}\\
& & FQE (distributional) &$\bf 0.03$ & $\bf {\scriptstyle \, \pm 0.03}$ & $\bf 0.01$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\bf 0.50$ & $\bf {\scriptstyle \, \pm 0.30}$ & $\color{dgray} 0.73$ & $\color{dgray} {\scriptstyle \, \pm 0.01}$ & \multicolumn{2}{c}{$0.11$}\\
& & Autoregressive Model &$\bf 0.04$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\bf 0.04$ & $\bf {\scriptstyle \, \pm 0.02}$ & $\color{dgray} 0.85$ & $\color{dgray} {\scriptstyle \, \pm 0.02}$ & $\bf 0.30$ & $\bf {\scriptstyle \, \pm 0.04}$ & \multicolumn{2}{c}{$0.04$}\\
 \bottomrule
 \end{tabular}
\caption{\label{tab:regret5}\small Normalized Regret@5 (bootstrap mean $\pm$ standard deviation) for OPE methods \vs{} ground truth values at a discount factor of $0.995$.
In each column, normalized regret values that are not significantly different from the best ($p >0.05$) are bold faced.
Methods are ordered by median.}
\end{center}  \end{table}
